SensorBench: Benchmarking LLMs in Coding-Based Sensor Processing

Effective processing, interpretation, and management of sensor data have emerged as a critical component of cyber-physical systems. Traditionally, processing sensor data requires profound theoretical knowledge and proficiency in signal-processing tools. However, recent works show that Large Language Models (LLMs) have promising capabilities in processing sensory data, suggesting their potential as copilots for developing sensing systems. To explore this potential, we construct a comprehensive benchmark, SensorBench, to establish a quantifiable objective. The benchmark incorporates diverse real-world sensor datasets for various tasks. The results show that while LLMs exhibit considerable proficiency in simpler tasks, they face inherent challenges in processing compositional tasks with parameter selections compared to engineering experts. Additionally, we investigate four prompting strategies for sensor processing and show that self-verification can outperform all other baselines in 48% of tasks. Our study provides a comprehensive benchmark and prompting analysis for future developments, paving the way toward an LLM-based sensor processing copilot.

==> 4_methodology.tex <==
\section{Self-verification Design and Analysis}\label{Sec:llmdsp}

% \xiaomin{Again, in section introducing the design, aviod using too much itemlize (itemlize can be used in evaluations). Instead, using either (1) First, second... (2) subsubsection.}

% \xiaomin{We should add more details in the design section (two to three pages). Make the below three components different subsubsection. Add more figures to illustrate if need.}
% \xiaomin{The design details are still not enough.}

\begin{figure}%[htbp]
    \centering
 \setlength{\abovecaptionskip}{0.cm}
    \setlength{\belowcaptionskip}{0.cm}
    % \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{figure/examples/algo_bd-DSP.drawio.pdf }
        % \caption{Verifier-aided \name}
        % \label{fig:va DSP}
    % \end{subfigure}
    \caption{Overview of \name. 
    % \xiaomin{Enlarge the figure and font size; Make it two-columns (width/height>1) and each component more clear}. 
    } 
    \label{fig:va DSP}
    \vspace{-1em}
\end{figure}

% As we conducted studies with the engineering experts, we observed a different mindset when solving the DSP benchmark - LLMs tend to handle the queries in one shot. Namely, LLMs neither inspect and understand the signal properties nor reflect on their own solutions. On the other hand, engineering experts solve the problem in an iterative manner:

% a comprehensive benchmark to evaluate the difficulty and complexity of various signal-processing tasks,
During our experiments with engineering experts, we observed a distinct approach to solving the benchmark, contrasting sharply with the methods employed by LLMs. Unlike LLMs, which tend to handle queries in a one-shot manner without a thorough inspection or reflection on the signal properties, engineering experts adopt a more iterative and reflective approach.

\textit{(1) Experts prioritize understanding the signals before processing queries.} They begin by visualizing the signals through graphs, performing spectrum analysis, and identifying unwanted noise interference or data deficiencies.

\textit{(2) Experts address challenges iteratively.} Although this approach requires significantly more time due to multiple iterations, they first propose tentative solutions to obtain initial feedback and then refine their strategies until satisfactory performance is achieved.


We thus adapt the existing self-verification approach \cite{shinn2024reflexion}, inspired by the expert problem solving process. We initialize three LLM-based modules: DSP Agent $M_a$, Verifier $M_v$, and Reflector $M_r$.



\begin{algorithm}[tbp]
\begin{algorithmic}[1]
\State Initialize DSP Agent, Verifier, Reflector: $M_a, M_v, M_{r}$. Initialize the task $q$ and input signal $g$. Let $n$ be the maximum self-verification round.
% \State Initialize policy $\pi_{\theta}(a_i|s_0), \theta = \{M_a, mem\}$
\State Random sample a DSP plan $\tau_0 = M_a(s_0, mem)$ and obtain inspection $i_0$ and output signal $o_0$
\State Let $s_0 = (q, g, i_0, \tau_0, o_0)$
\State Generate initial verification $v_0 = M_{v}(s_0, \tau_0)$
% \State Set $mem \leftarrow [sr_0]$
\State Set $t = 1$
% \If{$q \in \mathbb{S}$}
%     \State \textbf{return}
% \EndIf
\While{$v_0 == \text{False}$ and $t <= n$ trials}
    \State Generate $\tau_t = M_a(s_t, mem)$ and obtain $i_t$ and $o_t$
    \State Update $s_t = (q, g, i_t, \tau_t, o_t)$
    \State Evaluate $s_t$ by $v_t = M_{v}(s_t)$
    \State Generate self-reflection $r_t = M_{r}(s_t, v_t)$
    \State $mem \leftarrow (mem, r_t)$
    % \State $s_t = (q, g, i_t, \tau_t, o_t)$
    \State $t \leftarrow t + 1$
\EndWhile
\State \textbf{return}
\end{algorithmic}
\caption{\name}\label{algorithm}
\end{algorithm}

\noindent \textbf{Signal Properties Inspection.} First, the DSP Agent $M_a$ is required to implement an \textit{inspection} function to understand the properties of the signals. This initial step ensures that the $M_a$ comprehensively understands the signal's properties and the challenges that need to be addressed.

\noindent \textbf{LLM-guided self-verification.} In each iteration, once the DSP Agent $M_a$ performs a solution, the processed signal undergoes a verification process. We implemented a verifier module that asks the $M_v$ to perform sanity checks on the results. $M_v$ implements a sanity check tool that takes the processed and input signals as input and output pass or fail. These checks are designed to ensure that the solutions are logically consistent and meet the criteria proposed by the models. 

% Our design differs from existing self-verification works \cite{stechly2024self, yao2024tree, shinn2024reflexion} in two settings: (1) We ask the model to implement its own sanity check criteria explicitly instead of providing external verifiers for them. The reason is that in practical sensor processing, it is challenging for developers to propose criteria for diverse sensor processing tasks beforehand, thus limiting the generalization ability. (2) Our module $M_v$ is operated in a Python simulator instead of autonomous mode. The model writes a sanity check tool in Python instead of purely looking at the previous attempt. This helps the model perform sanity checks accurately and reduce hallucinations.

% \begin{figure}%[htbp]
%     \centering
%  \setlength{\abovecaptionskip}{0.cm}
%     \setlength{\belowcaptionskip}{0.cm}
%     % \begin{subfigure}[b]{0.45\textwidth}
%         \includegraphics[width=\linewidth]{figure/examples/algo_bd-verifier.drawio.pdf}
%     % \end{subfigure}
%     \caption{Verifier overview. A separate LLM is instructed to build a sanity check tool. The sanity check tool will take the input signal $g$ and processed signal $o_t$ as input and return pass or fail. } 
%     \label{fig:sanity_check}
% \end{figure}

\noindent \textbf{Memory-aided reflection.} If the solution fails the sanity checks, the process moves to the reflection phase. The results of the failed verification are passed to a reflector module $M_r$. The reflector $M_r$ is a stateful component with memory capabilities $mem$, allowing it to record previous failed attempts. This statefulness enables the reflector to build upon past experiences and provide more informed feedback. The verification result and the reflection are further concatenated with $mem$ and are passed on to the DSP agent $M_a$. 

The algorithm \ref{algorithm} explains the inspection, verification and reflection steps.

% Finally, we empirically observe that the model struggles to perform self-verification in tasks $\mathbb{Q} = \{\text{imputation}, \text{extrapolation}\}$. We thus set a rule-based verification switch - if the model frequently fails while performing self-verification for the task $q$ in $\mathbb{Q}$, i.e., $Pr(\text{verification fail for } $q$) >= 1 - \epsilon$, we explicitly set the number of self-verification rounds equal to 1 for the task. The rationale behind this approach is that when the model fails the self-verification with high probability, we think that the model cannot propose a useful verification criterion or the DSP agent is incompetent to pass the sanity check. Thus, $M_v$ and $M_r$ are disabled by setting $n=1$. We name this approach as \textbf{Ours (optimal)}.

==> 5_1_case_study.tex <==

\section{A Real-World Case Study: Monitoring of Respiration Signals with UWB Radar}\label{Sec:case_study}

% \VK{Case study can be a separate section after Results} 
% \subsubsection{Acoustic event detection}

% \subsubsection{HAR using IMUs}

% \subsubsection{Breath detection using mmWave radar}

% As radar technology advances, engineers have been using the technology to design remote sensing applications in health monitoring and surveillance \cite{zheng2020v2ifi, xie2023short, zheng2021more}.
In this section, we use a real-world case study to show the effectiveness of harnessing LLMs for signal processing.
% Compared to wearable sensors, contactless vital signal monitoring using UWB Radar is more comfortable and causes minimum interference to human subjects \cite{zheng2020v2ifi, xie2023short, zheng2021more}. Such methods are particularly useful in scenarios where contact-based methods are impractical, such as searching for vital signals in debris or health monitoring in vehicles. 
Specifically, we present the use of LLMs to perform noninvasive monitoring of vital signs using UWB Radar systems without the involvement of any engineering expert. 

In radar-based respiration monitoring, a radar system emits radio waves and captures the reflected signals. When a subject is present within the Radar's range, their movements, including respiration, modulate the reflected signals. These modulations can be analyzed to extract information about the subject's breathing patterns.
% dataset
In this case study, we employ a self-collected dataset to investigate the feasibility of employing LLMs to recover vital signals from UWB Radar data. We instructed volunteers to sit relaxed at a fixed distance and collected datasets measured by the UWB Radar and a ground-truth respiration monitor. The collected Radar response is a complex matrix with two dimensions in time and distance, respectively. 

\begin{figure}%[htbp]
    \centering
 \setlength{\abovecaptionskip}{0.cm}
    \setlength{\belowcaptionskip}{0.cm}
        % \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.9\linewidth]{./figure/examples/respiration.png }
        % \caption{Inst}
    % \end{subfigure}
    \caption{Instruction prompt sent to GPT-4o. The remaining setup is the same as coding with APIs.}
    \label{fig:respiration-example}
    % \vspace{-1em}
\end{figure}

\begin{table}%[ht]
\centering
\resizebox{0.4\textwidth}{!}{%
\LARGE
\begin{tabular}{llr}
\toprule
 Metric & GPT-4o & Zheng et al. \cite{zheng2020v2ifi} \\
 \midrule
 $\downarrow$ Distance error (m) & $0.11 \pm 0.41$ & $0.08 \pm 0.03$\\
\midrule
$\uparrow$ Correlation & $0.32\pm0.19$ & $0.38\pm0.21$ \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of using GPT-4o and Zheng et al \cite{zheng2020v2ifi} in respiration monitoring with UWB Radar.}
% Distance error measures the difference between the estimated distance and the ground-truth distance of the subject. Correlation measures the linear relationship between the recovered trace and the ground-truth respiration trace.
\label{table:uwb_res}
\vspace{-2em}
\end{table}





% We refer our readers to Appendix \ref{uwb_radar} for the detailed data explanation and data collection protocol. 

Similar to the base method described in Sec. \ref{appendix:settings}, we instructed GPT-4o to recover respiration traces from radar signals, where the model is allowed to call Python APIs for problem-solving. We provided the model with the proper context as shown in Fig. \ref{fig:respiration-example}. In this setup, we did not provide the location of the subject or any prior knowledge of DSP to the model. Instead, the model was instructed to estimate the distance bin that best represents the subject's location. 

Based on the setup, we calculate an estimated distance from the object to the Radar as the ground truth location. We evaluated the model's performance using the absolute error in estimating the subject's distance. Additionally, we assessed the quality of the recovered respiration signal by measuring the absolute correlation between the radar signal at the estimated distance and the ground-truth respiration trace. The results provided by GPT-4o are compared with that of Zheng et al \cite{zheng2020v2ifi}, where GPT-4o normally uses spectrum analysis to identify the possible location.



Table \ref{table:uwb_res} shows the overall performance of both approaches.  We evaluate the pipelines on two volunteers over a total duration of 10 minutes of collected data. The model processes a 30-second Radar matrix at a time, with 3 random repetitions, resulting in 60 different trials. The results indicate that GPT-4o's performance is comparable to the expert's solution in both distance error and correlation metrics. Besides, we visualize the respiration traces recovered by both approaches in Fig. \ref{fig:case_study_vis}, which shows that the recovered traces closely resemble the ground-truth traces produced by the respiration monitor. This case study demonstrates the potential of using LLMs in real-world DSP problems, making them more accessible to non-experts.


\begin{figure}%[htbp]
    \centering
 \setlength{\abovecaptionskip}{0.cm}
    \setlength{\belowcaptionskip}{0.cm}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{./figure/case_study/39_gt.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{./figure/case_study/31_gt.png}
    \end{subfigure}
    \caption{Recovered traces by LLM and Zheng et al \cite{zheng2020v2ifi}.}
    \label{fig:case_study_vis}
    \vspace{-1em}
\end{figure}
% We leave an example code snippet produced by GPT-4o in Appendix \ref{uwb_radar}. 




==> 8_Ablation_study.tex <==
\subsection{Ablation Study}



\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
% \begin{tabular}{p{3cm}clllp{1.5cm}}
\begin{tabular}{lccccc}
\toprule
Task & Diff. & Base & ReAct & ReAct+In & ReAct+In+Verif (n=5) \\
\midrule
$\uparrow$ Change point detection & 4 & 0.1530 & 0.1621 & \underline{0.1957} & \textbf{0.2626} \\
$\uparrow$ Outlier detection & 4 & 0.2318 & 0.2575 & \textbf{0.4015} & \underline{0.3768} \\
$\uparrow$ Echo cancellation & 4 & \underline{2.9642} & \textbf{9.7490} & -1.4204 & -1.6403 \\
$\uparrow$ Speech Filtering & 4 & 6.4287 & \underline{6.8890} & 6.4737 & \textbf{9.7174} \\
\midrule
$\downarrow$ Delay detection & 2 & \textbf{0.0006} & 0.0091 & 0.1002 & \underline{0.0020} \\
$\downarrow$ ECG heartrate & 4  & 1546.0656 & \underline{667.8772} & 799.7044 & \textbf{36.2437} \\
$\downarrow$ Extrapolation & 3 & 24.8001 & \underline{0.3155} & \textbf{0.0854} & 1.2655 \\
$\downarrow$ ECG Filtering & 3 & 0.0016 & 0.0012 & \textbf{0.0002} & \underline{0.0007} \\
$\downarrow$ Imputation & 3 & 1.2245 & \textbf{0.1692} & \underline{0.5768} & 0.6246 \\
$\downarrow$ Period detection & 3 & 0.3661 & 0.3589 & \textbf{0.1516} & \underline{0.2139} \\
$\downarrow$ Resampling & 2 & \textbf{0.0003} & 0.1242 & \underline{0.0006} & 0.0366 \\
\midrule
Win rate (\%)  & - & 20 & 24 & 36 & 44 \\
\bottomrule
\end{tabular}
}
\caption{Ablation study. The variations include base, ReAct \cite{yao2022react}, ReAct + Inspection ($n=1$), and ReAct + Inspection + Verification ($n=5$). The numbers in the first four rows of the table are the larger, the better. The best is made \textbf{bold}, and the second best is \underline{underscored}.}\label{table:performance_comparison_ablation_study}
\vspace{-2em}
\end{table}

In this section, we study the effectiveness of each design component in \name, i.e., the inspection module and self-verification module. Note that the reflection module is designed to reflect on the verification output, so we added reflection to the verification module in this study. 

Table \ref{table:performance_comparison_ablation_study} shows the performance of different combinations of the design components. The variations include base, ReAct \cite{yao2022react}, ReAct + Inspection ($n=1$), and ReAct + Inspection + Verification ($n=5$). Comparing ReAct \cite{yao2022react} with ReAct + Inspection, we could observe that adding the inspection module significantly helps improve the performance of LLM in Change point detection, Outlier detection, ECG filtering, Resampling, and Period detection. This demonstrates that inspection helps understand the problem landscape and design an appropriate plan. 

Besides, without self-verification, the setting of ReAct + Inspection underperforms ReAct + Inspection + Verification $n=5$ in the most difficult compositional tasks (Diff. $=4$), such as Change point detection, Spectral filtering-speech, and Heart rate calculation. This observation supports our hypothesis that iterative self-verification is more beneficial for tasks that require multi-step planning and parameter selection since it allows models to perform with trial and error. With verification, the model achieves the highest win rate 44\% in all tasks.

% \begin{figure*}[htbp]
%     \centering

%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Change point detection.png}
%         \caption{Change point detection}
%         \label{fig:change_point_detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Filtering Speech.png}
%         \caption{Spectral filtering-speech}
%         \label{fig:echo_cancellation}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Outlier detection.png}
%         \caption{Outlier detection}
%         \label{fig:outlier_detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Echo cancellation}
%         \caption{Echo cancellation}
%         \label{fig:filtering_speech}
%     \end{subfigure}

%         \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Filtering ECG.png}
%         \caption{Spectral filtering-ECG}
%         \label{fig:change_point_detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_ECG heartrate .png}
%         \caption{Heart rate calculation}
%         \label{fig:echo_cancellation}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Resampling.png}
%         \caption{Resampling}
%         \label{fig:outlier_detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Period detection.png}
%         \caption{Period detection}
%         \label{fig:filtering_speech}
%     \end{subfigure}

%         \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Delay detection.png}
%         \caption{Delay detection}
%         \label{fig:change_point_detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Imputation.png}
%         \caption{Imputation}
%         \label{fig:echo_cancellation}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[width=\textwidth]{./figure/abl_std/n_Extrapolation.png}
%         \caption{Extrapolation}
%         \label{fig:outlier_detection}
%     \end{subfigure}


%     \caption{Performance Comparison for Various Tasks. The variations include base, ReAct \cite{yao2022react}, ReAct + Inspection ($n=1$), and ReAct + Inspection + Verification ($n=5$). Filtering Speech, Echo cancellation, Change point detection, Outlier detection, and Echo cancellation (the first row) are the larger the better; the remaining tasks are the smaller the better.}
%     \label{fig:performance_comparison_ablation_study}
    
% \end{figure*}


% \begin{table}[ht]
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{p{3cm}lllp{1.5cm}}
% \toprule
% Task & Base & ReAct & ReAct+In & ReAct+In+Verif (n=5) \\
% \midrule
% $\uparrow$ Change point detection & 0.1530 & 0.1621 & \underline{0.1957} & \textbf{0.2626} \\
% $\uparrow$ Outlier detection & 0.2318 & 0.2575 & \textbf{0.4015} & \underline{0.3768} \\
% $\uparrow$ Echo cancellation & \underline{2.9642} & \textbf{9.7490} & -1.4204 & -1.6403 \\
% $\uparrow$ Filtering Speech & 6.4287 & \underline{6.8890} & 6.4737 & \textbf{9.7174} \\
% \midrule
% $\downarrow$ Delay detection & \textbf{0.0006} & 0.0091 & 0.1002 & \underline{0.0020} \\
% $\downarrow$ ECG heartrate  & 1546.0656 & \underline{667.8772} & 799.7044 & \textbf{36.2437} \\
% $\downarrow$ Extrapolation & 24.8001 & \underline{0.3155} & \textbf{0.0854} & 1.2655 \\
% $\downarrow$ Filtering ECG & 0.0016 & 0.0012 & \textbf{0.0002} & \underline{0.0007} \\
% $\downarrow$ Imputation & 1.2245 & \textbf{0.1692} & \underline{0.5768} & 0.6246 \\
% $\downarrow$ Period detection & 0.3661 & 0.3589 & \textbf{0.1516} & \underline{0.2139} \\
% $\downarrow$ Resampling & \textbf{0.0003} & 0.1242 & \underline{0.0006} & 0.0366 \\
% \midrule
% Win rate (\%)  & 20 & 24 & 36 & 44 \\
% \bottomrule

% \end{tabular}

% }

% \caption{Ablation study. The variations include base, ReAct \cite{yao2022react}, ReAct + Inspection ($n=1$), and ReAct + Inspection + Verification ($n=5$). Filtering Speech, Echo cancellation, Change point detection, Outlier detection, and Echo cancellation (the first part of the table) are the larger the better; the remaining tasks are the smaller the better.}\label{table:performance_comparison_ablation_study}
% \end{table}


% \begin{figure*}[htbp]
%     \centering
%  \setlength{\abovecaptionskip}{0.cm}
%     \setlength{\belowcaptionskip}{0.cm}
%         \begin{subfigure}[b]{0.30\textwidth}
%         \includegraphics[width=\textwidth]{./figure/examples/imp.png}
%         \caption{Imputation}
%         \label{fig:Delay detection}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.29\textwidth}
%         \includegraphics[width=\textwidth]{./figure/examples/ext.png}
%         \caption{Extrapolation}
%         \label{fig:echo_cancellation}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.30\textwidth}
%         \includegraphics[width=\textwidth]{./figure/examples/echo.png}
%         \caption{Adaptive filtering}
%         \label{fig:outlier_detection}
%     \end{subfigure}
%     \caption{Self-verification criteria proposed on imputation, extrapolation, and adaptive filtering. These criteria may not be valid and even misleading.}
%     \label{fig:verf-example}\vspace{-1em}
% \end{figure*}

\begin{figure}[htbp]
    \centering
 \setlength{\abovecaptionskip}{0.cm}
    \setlength{\belowcaptionskip}{0.cm}
        \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./figure/examples/imp.png}
    \end{subfigure}
    \caption{Self-verification criteria proposed on imputation. The criteria may not be valid and even misleading.}
    \label{fig:verf-example}\vspace{-1em}
\end{figure}

\begin{figure}%[htbp]
    \centering
 \setlength{\abovecaptionskip}{0.cm}
    \setlength{\belowcaptionskip}{0.cm}
        \includegraphics[width=\linewidth]{figure/Pearson-taskwise.pdf}
    \caption{Pearson coefficient between the number of self-verification rounds and absolute performance of different tasks. A positive Pearson coefficient indicates that the performance improves with more rounds of self-verification.}\label{fig:pearson}
    \vspace{-1em}
\end{figure}


\subsection{Impact of Self-verification}\label{Sec:impact-self-verif} 
In this section, we study the impact of the number of self-verification round in \name. 


\subsubsection{Correlation between Model Performance and Number of Self-verification Rounds} Figure \ref{fig:pearson} shows the Pearson correlation coefficient (defined as $r$) between the number of self-verification rounds ($n$) and the absolute performance of self-verification ($n=1$ to $5$). For tasks using MSE as an evaluation metric, we adopt its reciprocal as the absolute performance metric. Therefore, a positive Pearson coefficient indicates that the performance improves as the number of self-verification rounds increases. Statistically speaking, $|r|>=0.7$ indicates a strong correlation, $0.3 <= |r| < 0.7$ indicates a moderate correlation, while $|r| < 0.3$ indicates weak or no correlation.

As shown in Figure \ref{fig:pearson}, the performance of period detection, outlier detection, heart rate detection, and speech filtering have high to moderate positive correlations to the number of self-verification rounds. However, the performance of echo cancellation, imputation, and extrapolation exhibit negative correlations. This analysis underscores the varying effectiveness of the self-verification design across different tasks, suggesting that not all tasks will benefit from self-verification - if a task is challenging to verify even for domain experts, LLMs would also struggle to do self-verification.



The reasons why self-verification does not work on tasks such as imputation, extrapolation, and adaptive filtering are as follows. First, simple tasks such as linear imputation and statistical forecasting do not rely on multi-step planning. Instead, they only need to call one API without parameter selection, such as \texttt{np.interp} and \texttt{auto\_arima}. Thus, self-verification may cause the model to overthink. Second, self-verification is challenging for these tasks and is as complex as solving the problem. For example, it is difficult to define reliable criteria for imputation and extrapolation in extended signal reconstruction, i.e., verifying the validity of a solution is as technically hard as solving the problem. 
% Therefore, the model fails to propose a reasonable criterion for sanity check and thus leads to inferior performance through rejecting proper implementation. 

% Figure \ref{fig:verf-example} shows three examples where the model struggles to propose a suitable criterion for these tasks, thus reducing performance. In imputation, the model suggested using the closeness of mean and frequency of the imputed signal values as the criterion for sanity check. However, it arbitrarily picked a tolerance threshold of 0.01 without justification. In extrapolation, the model used a deviation tolerance of 0.1 for the prediction from the mean of the input signal. However, since the input data is an ECG signal, which naturally has peaks, this criterion is not appropriate. In adaptive filtering, the model used the closeness in dominant frequencies to indicate the success of echo removal. However, the dominant frequencies could be retained without any echo removal, rendering this criterion ineffective.

Figure \ref{fig:verf-example} shows an example where the model struggles to propose a suitable criterion for imputation tasks, thus reducing performance. In imputation, the model suggested using the closeness of mean and frequency of the imputed signal values as the criterion for sanity check. However, it arbitrarily picked a tolerance threshold of 0.01 without justification. The criteria may not be valid and even misleading.

\subsubsection{Performance Changes with Varying Numbers of Self-verification Rounds} Table \ref{table:performance_comparison_n} shows the performance changes when performing different rounds of self-verification over the base prompting approach on GPT-4o. In this evaluation, the model performs self-verification on all tasks (including imputation and extrapolation) using $n=3$, $4$, and $5$. The results indicate a consistent trend across all $n$ values. Self-verification surpasses the baseline on most tasks, such as change point detection, speech filtering, outlier detection, and heart rate calculation. The only exception is echo cancellation, where using self-verification consistently results in worse performance. Additionally, in delay detection and resampling, the base approach performs exceptionally well (7900\% and 87400\% better than expert 2, respectively). Thus, the performance for $n=3$, $4$, and $5$ remains within a reasonable range.







\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrr}
\toprule
Task & n=3 (\%) & n=4 (\%) & n=5 (\%) \\
\midrule
$\uparrow$ Change point detection & +76.7 & +85.1 & +71.7 \\
$\uparrow$ Outlier detection  & +39.0 & +28.6 & +62.6 \\
$\uparrow$ Echo cancellation  & -191.8 & -277.1 & -155.3 \\
$\uparrow$ Speech Filtering & +25.6 & +9.9 & +51.2 \\
\midrule
$\downarrow$ Delay detection & -77.3 & +1178.7 & +218.0 \\
$\downarrow$ ECG heart rate & -68.5 & -74.8 & -97.7 \\
$\downarrow$ Extrapolation  & -99.3 & -94.4 & -94.9 \\
$\downarrow$ ECG Filtering  & -7.0 & -90.0 & -56.2 \\
$\downarrow$ Imputation & -50.9 & -22.7 & -49.0 \\
$\downarrow$ Period detection & -69.0 & -87.0 & -41.6 \\
$\downarrow$ Resampling & +27184.5 & +10000.0 & +10562.1 \\
\bottomrule
\end{tabular}
}
\caption{Comparing different numbers of self-verification rounds ($n$). We calculate the performance change against the base approach. The first four rows are the higher, the better.}\label{table:performance_comparison_n}
% \vspace{-2em}
\end{table}

% Base on the above study, we summarize our answer to Q3 as below:

% \begin{tcolorbox}[colframe=black, colback=white, title=\textbf{Answer to Q3}]
% Self-verification improves the LLMs' performance on a majority of tasks compared to SOTA. The exceptions are the tasks that are challenging to define criteria, e.g., imputation, extrapolation, and echo cancellation.
% \end{tcolorbox}

In summary, base on the above study, we can conclude that self-verification improves the LLMs' performance on a majority of tasks compared to SOTA. The exceptions are the tasks that are challenging to define verification criteria, e.g., imputation, extrapolation, and echo cancellation.
